The Simons Observatory: laboratory beam characterization for the first small aperture telescope

The Simons Observatory is a ground-based telescope array located at an elevation of 5200 meters, in the Atacama Desert in Chile, designed to measure the temperature and polarization of the cosmic microwave background. It comprises four telescopes: three 0.42-meter small aperture telescopes (SATs), focused on searching for primordial gravitational waves, and one 6-meter large aperture telescope, focused on studying small-scale perturbations. Each of the SATs will field over 12,000 TES bolometers, with two SATs sensitive to both 90 and 150GHz frequency bands (SAT-MF1, and SAT-MF2), while the third SAT is sensitive to 220 and 280GHz frequency bands. Prior to its deployment in 2023, the optical properties of SAT-MF1 were characterized in the laboratory. We report on measurements of near-field beam maps acquired using a thermal source along with measurements using a holographic method that enables characterization of the amplitude and phase of the beam response, yielding an estimate of the far-field radiation pattern received by SAT-MF1. We find that the near-field half-width-half-maximum (HWHM) requirements are met across the focal plane array for the 90GHz frequency band, and through most of the focal plane array for the 150GHz frequency band. The mean of the bandpass averaged HWHM of the edge-detector focal plane modules match the simulated HWHM to 10.4%, with the discrepancy caused by fringing in the simulation. The measured beam profiles match simulations to within 2dB from the beam center to at least the -10dB level. Holography estimates of the far-field 90GHz beams match the full-width-half-maximum from simulation within 1%, and the beam profiles deviate by less than 2dB inside the central lobe. The success of the holography and thermal beam map experiments confirmed the optical performance was sufficient to meet the science requirements. On-site observations are currently underway.

==> sections/scratch_writing/introduction.tex <==
% \begin{itemize}
%   \item SO + CMB Background
%     \begin{itemize}
%         \item The Simons Observatory (SO) is an array of four telescopes dedicated to observing the temperature and polarization signals of the cosmic microwave background (CMB). 
%         \item Why characterize beams?
%     \end{itemize}
%   \item SAT-1 Optical Design
%     \begin{itemize}
%         \item Sentences here
%     \end{itemize}
%   \item Short history of beam map collection practices
%     \begin{itemize}
%         \item Sentences here
%     \end{itemize}
%   \item MAYBE: Include SAT Optics goals (beam size, ellipticity, etc.) <Ref SO science goals?>
%     \begin{itemize}
%         \item Sentences here
%     \end{itemize}
% \end{itemize}
    Intensity only (thermal) beam maps are used in cosmology as confirmation and calibration of telescope optics, testing the angular response of the telescope as the intensity source scans across the focal plane's field of view. Characterizing the beam shape, specifically the full-width-half-max (FWHM), ellipticity, and side-lobes allows cosmologists to accurately deconvolve \cite{beam_characteristics} the telescope beam from the observed CMB sky \cite{beam_leakage}, \cite{Duivenvoorden_2019}. 
    
    Ideally, cosmologists would create far-field intensity beam maps before deploying the telescope to site. However, running far-field tests in lab is a challenging task: light pollution, air pollution, and atmospheric turbulence makes accurately creating beam maps near impossible. Cosmologists create near-field thermal beam maps for a first-order test of the telescope optics. Systematics in the observed beam can be learned and accounted for, allowing for cosmologists to repair and retrofit the telescope in lab, a much easier task than doing so in the Atacama Desert. 
    Collaborators at the University of Chicago in 2021 applied the holographic method to measure the near-field beam intensity and polarization of the LAT-test receiver optics tube, allowing them to estimate the far-field beam response of the telescope \cite{Chesmore_2022}, \cite{near-field_holog}. From late 2022 to early 2023, I helped develop and test near-field thermal and holography beam maps for SAT-MF1 at University of California San Diego (UCSD) with the UChicago collaborators and UCSD team members. 
    
    Our experiments confirmed SAT-MF1 optics meet requirements, namely the mean of the bandpass averaged FWHM matches simulated FWHM, 34.5m for 90GHz and 28.2cm for 150GHz frequency bands within 3$\%$ (90GHz) and within 9$\%$ at 150 GHz. The measured radial profile of the beams matches simulations to within 2dB from the beam center to at least the -10dB level. Holography estimates of the far-field 90 GHz beams match simulations to within 10$\%$. The success of the holography and thermal beam map experiments allowed us to deploy SAT-MF1 in June, 2023. On-site observations are currently underway. 



\begin{figure}[ht!]
    \centering
    \includegraphics[height=6cm]{figures/sat1_fpa.png}
    \includegraphics[height=6cm]{figures/ticra_near-field_sims.png}
    \caption{Left: Focal Plane of SAT-MF1. Note, Mv7 (bottom left) was excluded from thermal beam map analysis {\bf\textcolor{red} {[say why]}}. Green text boxes: Names of Universal Focal-plane Modules (UFMs) without a rhombus blocking off 1/3 of detectors. Black rhombuses: Blocked off detectors via copper rhombus attached to UFM. Blue text boxes: Names of UFMs with a rhombus blocking off 1/3 detectors. Stars: Locations of holography readout sensors. Right: \textbf{Ticra Tools} model and simulation of the thermal beam and holography setup using SAT-MF1 optics. The holography source was 39cm from the aperture stop of SAT-MF1, and the thermal beam source was 81cm from the aperture stop of SAT-MF1. Right side: Pixels on the focal plane, blue lines go to a pixel at a radial distance of 16.3cm from the center of the focal plane. Red lines go to a pixel at the center of the focal plane. Pink plane: the aperture stop of SAT-MF1. Light blue planes: Planes from which beam sources are emitted.}
    \label{fig:sat_fpa}
\end{figure}

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=7cm]{figures/ticra_near-field_sims.png}
%     \caption{\textbf{Ticra Tools} model and simulation of the thermal beam and holography setup using SAT-MF1 optics. The holography source was 39cm from the aperture stop of SAT-MF1, and the thermal beam source was 81cm from the aperture stop of SAT-MF1. Right side: Pixels on the focal plane, blue lines go to a pixel at a radial distance of 16.3cm from the center of the focal plane. Red lines go to a pixel at the center of the focal plane. Pink plane: the aperture stop of SAT-MF1. Light blue planes: Planes from which beam sources are emitted.}
%     \label{fig:near_field_optics}
% \end{figure}


==> sections/scratch_writing/thermal_pipeline.tex <==
    \begin{figure}[ht!]
        \centering\includegraphics[width=7cm,height=5cm]{figures/mv14_both_beams.jpg}
        \caption{Observed beam maps after data processing. Left: 90GHz beam on a central pixel with power slices through the center of the beam. Right: 150GHz beam on a central pixel with power slices through the center of the beam.}
        \label{fig:central_thermal_beams}
    \end{figure}

   In this section, we detail the analysis pipeline and the methods used to analyze our beams and compare them to simulations. First, we discuss the simulation software used to simulate the SAT-1 near-field thermal beams, Ticra Tools\footnote{\url{https://www.ticra.com/}}. Second, we discuss the pre-processing pipeline that is used to produce beam maps from time-ordered-data (TOD). Lastly, we discuss the algorithms used to compare the simulated beam radial profiles to the observed SNR-weighted average beam radial profiles.

   Using Ticra Tools, we simulate the SAT-1 optical response to the near-field thermal source by calculating the electric field through each optical interface. Fig~\ref{fig:near_field_optics} depicts the simulation setup along with the optical components in SAT-1. The optics contain three refractive lenses, an aperture stop, feedhorns, and the focal plane. This simulation includes two planes of emission: 81cm from the aperture stop, corresponding to the near-field thermal beams; and 39cm from the aperture stop, corresponding to the holography near-field beam maps. Beam maps are simulated at two positions in the focal plane: one at the center of the focal plane; and the other at the edge of the focal plane, at a radial distance of 16.9cm from the center.   Ticra Tool simulations calculate beam radial profiles from monochromatic sources, thus we average simulated beam maps across observing frequency bands to compare with the observed thermal beam maps. We weight the intensity in each simulated beam map by the transmissivity of the neutral density filters (NDFs) placed in front of the TES bolometers inside SAT-MF1. \warn{Plot or reference NDF transmissivity?} 
   
    The first step in the analysis pipeline is to pre-process each of the detector TODs by lineraly detrending the timestream data and passing it through a 4th order high-pass butterworth filter with 2Hz cutoff frequency {(\bf\textcolor{orange}{Reference sotodlib paper})}. The TODs are then demodulated at the chop frequency (10Hz), the x/y stage positions are mapped to the timestamps in the the detector timestreams, and the amplitude of the detected signal at each pixel in the beam map is computed as the average value of the TOD over the 0.5s integration time. 
    
    \begin{figure}[ht!]
        \centering
        \includegraphics[width=7cm]{figures/cleaned_beam_ex.png}
        \caption{Observed beam maps before and after cleaning. Top: Before cleaning, the red 10x10 cm square encompasses the brightest pixel. Bottom: After cleaning, red square encompasses the brightest pixel after the previous brightest pixel was masked out. \warn{Ignore the orange square}}
        \label{fig:cleaned_beam}
    \end{figure}

    \begin{figure}[ht!]
        \centering
        \includegraphics[width=7cm,height=4cm]{figures/centroid_found.png}
        \caption{Observed beam map after cleaning. Red circle depicts 7.5cm radius circle used to calculate the average signal within the circle.}
        \label{fig:centroid_found}
    \end{figure}

    \begin{figure}[ht!]
        \centering
        \includegraphics[width=7cm,height=4cm]{figures/final_ellipse_fit.png}
        \caption{Observed beam map after cleaning and smoothing the main beam max signal. Red circle is the results of the fitted ellipse with the major axis as the radius.}
        \label{fig:final_ellipse_fit}
    \end{figure}

 {[\bf\textcolor{blue}{Remy begins re-writing here}]}

    The next step in the analysis pipeline is to remove sporadic noise from the observed beam map data. The pixel with maximum observed signal is removed if its observed intensity is {$\ge3\sigma$} than the average intensity within a 10x10 cm square surrounding it. Fig~\ref{fig:cleaned_beam} provides an example of removing a sporadic pixel. We then fit for the centroid of the observed beam maps for the 90GHz and 150GHz detectors using two different methods.

    \begin{figure}[ht!]
        \centering
        \includegraphics[width=7cm,height=4cm]{figures/150_ghz_beam_fit.png}
        \caption{150GHz beam with 2D Gaussian fit overplotted. Blue curve is a power slice across the horizontal and vertical axes of the beam. Orange is horizontal and vertical power slices of the 2D Gaussian fit.}
        \label{fig:150_gauss_fit}
    \end{figure}

    First, we discuss fitting the centroid of the observed beams for detectors within the 150GHz bandpass. The observed beams  are non-Gaussian below -5dB due to the aperture stop cutting off signal past 21cm from the center of the beam, an example can be seen on the right panel of figure ~\ref{fig:central_thermal_beams}. To account for this, we implement a weighted fitting of a 2D Gaussian \warn{(ref 2D Gaussian equation)} to the observed beam map. The weights are the inverse of the observed intensity. We then use the fitted centroid as the center of the observed beam in the 150 GHz passband detectors.

    Next we discuss fitting detectors in the 90 GHz passband. These detectors did not observe Gaussian near-field beams  because the 90 GHz detectors were over-saturated, in addition to the 42 cm aperture stop cutting off lower power signal. This produces a relatively flat beam with sharp cutoffs 21 cm away from the beam center (left panel of figure ~\ref{fig:central_thermal_beams}). To account for the flat-top shape of the 90 GHz beams, we implement an ellipse fitting and re-fitting algorithm to find the beam centroid.  The first ellipse is fit over all pixels that observe a signal power $\ge -3 dB$ from the maximum signal in the beam map. The bottom panel of figure ~\ref{fig:cleaned_beam} approximates the location of the maximum signal pixel (red box). We then calculate the average power within a 7.5cm radius circle around the fitted ellipse centroid (figure ~\ref{fig:centroid_found}), and re-fit an ellipse to all pixels that observe at least half of the average power around the center of the beam (figure \ref{fig:final_ellipse_fit}.  The averaging smoothes the observed beam and provides a more accurate location of the center of the beam. Thus, we use the center calculated from the second ellipse fit as the center of the observed beam in the 90 GHz passband detectors.   

    \begin{figure}[ht!]
        \centering
        \includegraphics[width=7cm,height=5cm]{figures/stacked_mv14_beams.jpg}
        \caption{Stacked beams on the central UFM, Mv14. Beams are averaged with SNR-weighting and beams that did not see a beam or produced unphysical fits are omitted. Left Panel: Stacked 90GHz detector beam. Right Panel: Stacked 150GHz detector beam.}
        \label{fig:stacked_beams}
    \end{figure}

    Comparisons between observed beam maps and simulated beam maps are done using the radial profiles of composite beams as done in \cite{BK11}. The metrics of comparison are provided by \warn{Ref SO-SAT Testing Document} and are the half-width half-max (HWHM), and the deviation in beam power up to -10dB of the simulated beam. Composite beams provide a measure of the optical performance across the focal plane array (FPA), and the beam radial profile ensures direct comparison with simulation. We calculate composite beam maps from an SNR-weighted average of all detectors within the 90 and 150 GHz frequency bandpasses within a UFM. Detectors that were dark or failed to be accurately fit did not contribute to the composite beam map. Figure~\ref{fig:sat_fpa} depicts the FPA and calls out the locations of each UFM in SAT-MF1. Thus, to make comparisons to the Ticra Tools simulation, we created composite beam maps in the 90 and 150 GHz frequency bandpasses using UFMs at the center of the FPA (Mv14), and at the edge of the FPA (Mv19). Fig~\ref{fig:stacked_beams} depicts the composite beam maps for UFM Mv14 in the 90GHz (left panel) and 150GHz (right panel) frequency bandpasses. 

 {[\bf\textcolor{blue}{Remy ends re-writing here}]}


==> sections/scratch_writing/thermal_results.tex <==
\subsection{Thermal Beam Results}
    \begin{figure}[ht!]
        \centering
        \includegraphics[scale=0.3]{figures/central_pixel_90GHz_radial_beam_profile.png}
        \includegraphics[scale=0.3]{figures/central_pixel_90GHz_beam_deviation.png}
        \includegraphics[scale=0.3]{figures/central_pixel_150GHz_radial_beam_profile.png}
        \includegraphics[scale=0.3]{figures/central_pixel_150GHz_beam_deviation.png}
    
        \caption{Near-field thermal beam profiles for the central UFM (Mv14). Top: 90GHz beam analysis. Left panel is the radial beam profile of the composite beam (blue) versus the simulated beam profile (red). The HWHM is the radial distance at which the beam power crosses -3dB. Right panel is the beam power deviation within the central beam. The deviation must be $<2 dB$ up to $-10 dB$ of the simulated beam. Bottom: 150GHz beam analysis. Left panel is the observed thermal beam (blue) versus the simulated band pass averaged beam (red). Right panel is the beam power deviation within the central beam.}
        \label{fig:mv14_near-field_profile}
    \end{figure}

    \begin{figure}[ht!]
        \centering
        \includegraphics[scale=0.3]{figures/edge_pixel_90GHz_radial_beam_profile.png}
        \includegraphics[scale=0.3]{figures/edge_pixel_90GHz_beam_deviation.png}
        \includegraphics[scale=0.3]{figures/edge_pixel_150GHz_radial_beam_profile.png}
        \includegraphics[scale=0.3]{figures/edge_pixel_150GHz_beam_deviation.png}
    
        \caption{Near-field thermal beam profiles for UFMs on the radial edge of the FPA. Top: 90GHz beam analysis. Left panel is the radial beam profile of the composite beam (blue) versus the simulated beam profile (red). The HWHM is the radial distance at which the beam power crosses -3dB. Right panel is the beam power deviation within the central beam. The deviation must be $<2 dB$ up to $-10 dB$ of the simulated beam. Bottom: 150GHz beam analysis. Left panel is the observed thermal beam (blue) versus the simulated band pass averaged beam (red). Right panel is the beam power deviation within the central beam.}
        \label{fig:mv22_near-field_profile}
    \end{figure}
 
    Figures ~\ref{fig:mv14_near-field_profile} and ~\ref{fig:mv22_near-field_profile} show the deviation of the observed beam from the simulated beam for both MF-1 and MF-2 at the center and edge of the focal plane, respectively. The center-pixel beam deviations of both MF-1 and MF-2 remain  below 2dB up to -10dB of the simulated beam, and are thus compliant with the SAT-MF1 testing requirements. The feature at approximately 18cm in the 150 GHz beam deviation can be explained by fringing in the MF-2 simulation, as we have only a simulation at only one frequency (150 GHz) at the time of this writing. The deviation between observed beams and simulated beams at the edge of the FPA remain within specifications as well.

    The HWHMs from the observed and simulated thermal beams at the center (Mv14) and averaged around the edge of the FPA, along with the experimental error between the two, are listed in table ~\ref{tab:hwhm_comparisons}. The HWHM is defined as the radial distance from the center of the beam to the point the beam crosses -3dB in power. In Mv14, the 90GHz passband observed the HWHM to be 17.5 cm, while the simulated HWHM is 17.9 cm, agreement within 3$\%$. In the 150 GHz passband, the observed HWHM is 13.5 cm, while the simulated HWHM is 14.2cm, agreement within 5 $\%$ of simulation. For the edge pixels in MF-1, the observed thermal beam HWHM is 17.9 cm, and the simulated HWHM is 17.8 cm, agreement within $1\%$. For MF-2, the observed thermal beam HWHM is 14.9 cm, and the simulated HWHM is 13.5 cm, agreement within $11\%$. The monotonically increasing deviation between observed and simulated beam radial profiles observed in all UFMs and across both bandpasses is due to the increased noise in the laboratory setting compared to simulations.

    \begin{table}[ht]
        \centering
        \begin{tabular}{|c|c|c|c|}
        \hline
             Parameter & Design Value (cm) & Measured Value (cm) & Error ($\%$) \\
             \hline
             Central HWHM 90GHz & $17.9 \pm 0.7$ & $17.5 \pm 0.23$ & 2.2 \\
             Edge HWHM 90GHz & $17.9 \pm 0.7$ & $17.8 \pm 0.05$ & 0.6 \\
             Central HWHM 150GHz & $14.2 \pm 1.58$ & $13.5 \pm 0.62$ & 4.9 \\
             Edge HWHM 150GHz & $13.5 \pm 0.7$ & $14.9 \pm 0.88$ & 10.4 \\
        \hline
        \end{tabular}
        \caption{Table of simulated HWHM and observed HWHM for central and edge pixels of 90 and 150GHz bandpasses}
        \label{tab:hwhm_comparisons}
    \end{table}

    % \begin{table}[ht]
    %     \centering
    %     \begin{tabular}{|c|c|c|c|}
    %     \hline
    %          Parameter & Design Value (cm) & Measured Value (cm) & Error ($\%$) \\
    %          \hline
    %          Central HWHM 90GHz & $17.9 \pm 0.8$ & $17.5 \pm 0.82$ & 2.2 \\
    %          Edge HWHM 90GHz & $17.9 \pm 0.8$ & $17.8 \pm 0.8$ & 0.6 \\
    %          Central HWHM 150GHz & $14.2 \pm 1.6$ & $13.5 \pm 0.62$ & 4.9 \\
    %          Edge HWHM 150GHz & $13.5 \pm 0.7$ & $14.9 \pm 0.88$ & 10.4 \\
    %     \hline
    %     \end{tabular}
    %     \caption{Table of simulated HWHM and observed HWHM for central and edge pixels of 90 and 150GHz bandpasses}
    %     \label{tab:hwhm_comparisons}
    % \end{table}




    \subsection{Holography Results}
    
    \begin{figure}[ht!]
        \centering
        \includegraphics[scale=0.4]{figures/90_farfield_beams.png}
        \caption{Band averaged 90GHz far-field estimation from holography measurements (left) and single frequency 90 GHz simulation from Ticra Tools (right).}
        \label{fig:farfield_prof}
    \end{figure}

    \begin{figure}
        \centering
        \includegraphics[scale=0.4]{figures/90_farfield_radial_profile.png}
        \caption{Far-field beam radial profile of the band-averaged 90 GHz holography estimate (black) and the simulated single frequency 90 GHz simulation (blue).}
        \label{fig:far-field-comps}
    \end{figure}

    For holography, the internal SO-SAT requirements document demands the estimated far-field response is compliant with 4 constraints: the MF-1 far-field response has FWHM of $< 30$ arcmin, the ellipticity of the beam is between 0.01 and 0.03, the integrated power within the center of the beam is $> 98\%$, and lastly, the central beam deviation is less than 2dB.
    
    The left panel of Figure \ref{fig:farfield_prof} is the MF-1 band averaged far-field beam response estimated holography measurements (85-115GHz), along with 1d cuts of power across the center of the beam. The right panel of Figure \ref{fig:farfield_prof} is the beam radial profile of the estimated MF-1 far-field beam. From the right panel, the integrated power in the near sidelobe region of the beam is $99\%$, and the central beam deviation is less than 2dB. The near sidelobe (central beam) and far sidelobe region are differentiated by 80 arcmin from the beam center, with the near sidelobe region within 80 arcmin, and the far sidelobe region outside 80 arcmin from the beam centroid. 

    The left panel of Figure ~\ref{fig:far-field-comps} compares individual frequency estimates of the far-field MF-1 beam response to the simulated beam response. The right panel (top) shows the FWHM (arcmin) in both x and y in arcmin per observed frequency. The bandpass averaged estimate of the MF-1 far-field FWHM is 27arcmin, $10\%$ smaller than the required 30 arcmin requirement.

    The ellipticity of the far-field responses in MF-1 are shown in Figure ~\ref{fig:far-field-comps} (right, bottom), with ellipticity defined as
    
    \begin{equation}
        \dfrac{\sigma_{max} - \sigma_{min}}{\sigma_{max} + \sigma_{min}}    
    \end{equation}
    , where $\sigma$ is the maximum or minimum spread of the fit 2D Gaussian. The ellipticity of the estimated far-field beam is not compliant with requirements, however the ellipticity is low enough to be handled in analysis and should not affect the sensitivity requirements of SO. We were unable to complete the 150GHz holography measurement due to scheduling constraints. 



==> sections/scratch_writing/thermal_setup.tex <==
    \subsection{Experimental Setup}
    In this section, we describe the experimental setup and data pipeline used to collect and analyze the near-field beam maps.

    \subsubsection{Near-Field Thermal Beam Experimental Setup}
    \begin{figure}[ht!]
        \centering
        \includegraphics[height=7cm]{figures/thermal_setup.jpg}
        \caption{Experimental setup for acquiring thermal beam maps. The 8020 scaffolding supports the X/Y stages and the heat source and chopper plate above the SAT. An Eccosorb blanket lies in the plane of the chopper plate to minimize reflections from electronics and the scaffolding. Note, SAT-MF1 is pointing at zenith.}
        \label{fig:thermal_setup}
    \end{figure}

   Design of the apparatus used to measure the near-field thermal beam maps of SAT-MF1 was guided by two primary considerations: the need to systematically scan a beam source across the viewing window and continuously monitor the measurement status; and the need to maximize the signal-to-noise ratio (SNR) of the beam signal as efficiently as possible.  
    
    Figure~\ref{fig:thermal_setup} shows the experimental setup during collection of the beam maps. The beam source used was a blackbody- emitting heater resistor attached to X/Y stages via a metal back-plate. The heater resistor was maintained at ~$760^\circ C$ and placed 81cm above the aperture stop of SAT-MF1. The X/Y stages are constrained to move in two dimensions and were held safely above SAT-MF1 by being bolted onto an Aluminum 8020 support structure. The beam source was moved in a 76x76cm square with 1cm resolution via raster scan, sufficient to measure at least twice the expected beam size. At a sample rate of 200Hz, the 0.5 sec integration time results in 100 data points per heat source position resulting in a map with SnR $\approx$ 50. Commanding and monitoring the position of the X/Y stages, and monitoring the temperature of the heat source, were all done via the Simons Observatory Control System (SOCS \cite{socs}). Current was sent through the source using a variac set by hand. 

    Reflections from the 8020 scaffolding and motors were mitigated by hanging a blanket lined with Eccosorb AN-72\footnote{\url{https://www.laird.com/products/absorbers/microwave-absorbing-foams/multi-layer-foams/eccosorb-an}} at ~300K in the field-of-view of SAT-MF1, with the beam source visible to the detectors through a 3.8cm aperture. To address long-timescale drifts, the source is modulated at 6 Hz using spinning fan blades covered in Eccosorb AN-72. The frequency of the dual-blade fan was monitored via an oscilloscope kept near SAT-MF1.

    To prevent the detectors from saturating, neutral density filters (NDFs) were installed onto the focal plane of SAT-MF1. The optical properties of the NDFs were studied in the paper, "The Simons Observatory:  In Lab Optical Testing and Validation for the First Small Aperture Telescope, SAT-MF1".   
    
    \subsubsection{Near-Field Holography Experimental Setup}
    \begin{figure}[ht!]
        \centering
        \includegraphics[scale=0.4]{figures/holography_source.jpg}
        \includegraphics[scale=0.13]{figures/holography_over_sat.jpg}
        \caption{Holography experimental setup. Left: Holography frequency source with waveguide. Right: Holography setup above the SAT-MF1 window with Eccosorb covering.}
        \label{fig:holography_source}
    \end{figure}
    
    The near-field holography source emits a monochromatic signal tuned to frequencies within the MF-1 (90 GHz) and MF-2 (150 GHz) bandpasses. We tuned the holography source to emit both co-polar and cross-polar signal at 5 GHz intervals over the frequency range of [85, 135] GHz using a waveguide twist to rotate the polarization of the signal by $90^{\circ}$. Scheduling constraints limited the number of single frequency beam maps tested, allowing only for frequencies within MF-1 (85 to 110 GHz) to be used in the analysis of this proceedings. This is because we compare the band-averaged far-field estimate of holography to simulation, and did not collect enough data for the MF-2 frequency band.       

    Section 3 of Chesmore et al \cite{Chesmore_2022} provides a schematic diagram of the holography source and receiver used for tuning. Similar to the thermal beam experimental setup, the holography source was also suspended above SAT-MF1 using the 8020 structure. We took 76x76cm beam maps at 1cm resolution. However, due the to size of the signal generator electronics and its attached waveguide, the holography source sat only 39 cm above the SAT-MF1 aperture stop compared to the 81cm distance separating the thermal heat source and the SAT-MF1 aperture stop. We used Eccosorb AN-72 to absorb reflections and radio signal from the holography electronics as shown in figure ~\ref{fig:holography_source}, and scanned the holography source across the field-of-view of SAT-MF1 using the same X/Y stages and motor controllers.    
    Eccosorb was wrapped only around the holography electronics as the signal-to-noise ratio (SNR) of the holography experiment was much greater than that of the thermal beam experiment. \textcolor{red}{I don't know if I would say that SNR is the reason we didn't use as much eccosorb. The real reason is a combination of (1) we've been more conservative in the past but haven't really found a super intense eccosorb necessary to get good data. and (2) I don't think you had the giant eccosorb blanket here at the time when we took holography. Maybe best to just not include that reason? I do think it's not as necessary for holography moreso due to the receiver and source only working with a single frequency and polarized source vs chromatic, unpolarized light. But could be that did add reflections in there.}
    
    There are three characteristics of the holography experimental setup that are distinct from the thermal beam map experimental setup. The holography signal is detected by a special purpose receiver, detailed in section 3.B in Chesmore et al. \cite{Chesmore_2022}), located at the radial edge of the focal plane (16.3 cm from center). Second, the the special purpose receiver is not at risk of saturating from the 300K background signal of the lab, so does not require the NDF. However, the 100mK detectors used within SAT-MF1 become saturated from the 300K background signal and require NDFs to mitigate the background signal. Lastly, the holography experiment requires the SAT focal plane to be cooled to 4K, rather than the operating temperature of 100mK used for the themal beam maps. This is because the special purpose receivers were not specified to operate at temperatures below 4K. \textcolor{red}{I would maybe still include a bit about how we need to be down to 4K vs say 40K so that the lenses are transmissive at our wavelengths}
